BiFlex: A Passive Bimodal Stiffness Flexible Wrist for Manipulation in Unstructured Environments

Robotic manipulation in unstructured, humancentric environments poses a dual challenge: achieving the precision need for delicate free-space operation while ensuring safety during unexpected contact events. Traditional wrists struggle to balance these demands, often relying on complex control schemes or complicated mechanical designs to mitigate potential damage from force overload. In response, we present BiFlex, a flexible robotic wrist that uses a soft buckling honeycomb structure to provides a natural bimodal stiffness response. The higher stiffness mode enables precise household object manipulation, while the lower stiffness mode provides the compliance needed to adapt to external forces. We design BiFlex to maintain a fingertip deflection of less than 1 cm while supporting loads up to 500g and create a BiFlex wrist for many grippers, including Panda, Robotiq, and BaRiFlex. We validate BiFlex under several real-world experimental evaluations, including surface wiping, precise pick-and-place, and grasping under environmental constraints. We demonstrate that BiFlex simplifies control while maintaining precise object manipulation and enhanced safety in real-world applications.

==> 06_Result.tex <==
\section{Result}
\label{s:result}

% \textcolor{blue}{Show off successful examples of solving the problems}

% 1. Performance Characterization Result
% \begin{itemize}
%     \item Show the variable stiffness curve graph with different flexible wrist. (Fig.~\ref{fig:Pressing_Test} 
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\columnwidth]{Figure/Drawing_Result_Instron.jpg}
%     \caption{Result for the Instron pressing test}
%     \label{fig:result_Instron}
% \end{figure}

% 2. Functional Validation Result
% \begin{itemize}
%     \item Present the pressing test results for three different grippers to validate the universality and interaction safety. (Fig.~\ref{fig:Result_PressingTest})
%     \item Present the wiping test results with the Robotiq gripper to validate the ease of control during interaction, thereby confirming performance at the interaction stage. (Fig.~\ref{fig:Result_WipingTest})
%     \item Present the pick-and-place test results with the Robotiq gripper to validate the manipulation performance, thereby confirming performance at the manipulation stage.(Table.~\ref{tab:pick_and_place_results})
% \end{itemize}


\subsection{Contacting Force Mitigation}



\subsection{Non-Flat Surface Adaptation}


\subsection{Precise Object Handling}










% \input{Table_tex/table_pressing_result}


% \input{Table_tex/table_pickandplace_result}



==> Backup.tex <==
% Inspired by human biomechanics, compliant end-effectors have been developed, demonstrating the ability to adapt to environmental conditions using simple actuation and control systems. These systems enable stable and natural interactions with the environment, yet the introduction of compliance raises a key challenge: while it enhances adaptability, it may compromise the ability to perform tasks that require precise control.

% To address this complexity, several studies have shown that humans adjust the stiffness of their limbs through muscular co-contraction to adapt to tasks with varying requirements \cite{}. Specifically, a higher stiffness is more effective in resisting perturbations and performing precision tasks, while a more compliant behavior is advantageous for tasks that involve exploring an unknown environment with minimal interaction forces.

% These features are typically facilitated by a wrist mechanism, which is usually an integral component of robotic and prosthetic arms. Despite its importance, much of the research in both academic and industrial settings has focused on advancing hand and gripper technologies, often overlooking the development of wrist systems \cite{}.

% \textcolor{blue}{What is the question we are trying to solve?}

% When a robotic hand interacts with its environment, high wrist compliance is crucial for stable and natural interactions, while high precision is important for fine-manipulation tasks. 
% However, most robot hands achieve compliance or precision, but not both. Although a rigid wrist design can achieve fine manipulation performance, it leads to poor interactions between the robotic hand and the environment. 
% This lack of compliance at the robotic wrist forces the robot manipulator to move slowly in pre-defined space and requires adding external sensors, which increases the computational load and complexity.
% On the other hand, a compliant wrist causes deflection, leading to position errors that deteriorate grasping performance. 
% Variable stiffness combine the benefit of both fields but require the additional active actuator with mechanism that increase the weight, size, and complexity. 
% Additionally, the limited \redst{durability} stiffness of soft materials restricts the wrist's compatibility, allowing it to handle only specific weight ranges. Therefore, complicated, actuator-dependent, and non-universal compliant wrists are difficult to implement in other robotic hands due to cost and maintenance challenges.

==> Figure_tex/fig_instron_pressing_test.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.35\columnwidth}
        \centering
        \begin{tikzpicture}
            % Include the image
            \node[anchor=south west, inner sep=0] (image) at (0,0) 
                {\includegraphics[trim={1cm 5cm 2cm 4.5cm}, clip, width=\linewidth]{Figure/Instron_Initial_Light_Grey.png}};
            
            % Scale coordinates to the image
            \begin{scope}[x={(image.south east)}, y={(image.north west)}]
                % Up Arrow 1
                \fill[color={rgb, 255:red, 139; green, 87; blue, 42}] 
                    (0.72, 0.68) -- (0.75, 0.61) -- (0.79, 0.68) -- (0.77, 0.68) -- 
                    (0.77, 0.76) -- (0.74, 0.76) -- (0.74, 0.68) -- cycle;
    
                % Up Arrow 2
                \fill[color={rgb, 255:red, 139; green, 87; blue, 42}] 
                    (0.79, 0.71) -- (0.82, 0.78) -- (0.86, 0.71) -- (0.84, 0.71) -- 
                    (0.84, 0.63) -- (0.81, 0.63) -- (0.81, 0.71) -- cycle;
    
                % Text Nodes
                \node[anchor=north west, font=\tiny] at (0.65, 0.63) {Loading};
                \node[anchor=north west, font=\tiny] at (0.75, 0.83) {Unloading};
            \end{scope}
        \end{tikzpicture}
        \caption{}
        \label{fig:Instron_initial}
    \end{subfigure}
    \begin{subfigure}[t]{0.57\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/Instron_Drawing.png}  
        \caption{} \label{fig:pressing_drawing}
    \end{subfigure}

    \caption{(a) Instron pressing system setup, and (b) free-body diagram illustrating how input sources (pressing force and deviation) are converted into joint torque and joint angle at the U-joint, thereby affecting the buckling behavior of the flexible wrist.}

    \label{fig:InstronPressingTest}
\end{figure}

==> Figure_tex/fig_pressing_test.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
       \includegraphics[width=1.0\textwidth]{Figure/FW_Pressing_Test_Robotiq1.png}
       \caption{}
       \label{fig:Pressing_Test1}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
       \includegraphics[width=1.0\textwidth]{Figure/FW_Pressing_Test_Robotiq2.png}
       \caption{}
       \label{fig:Pressing_Test2}
    \end{subfigure}
    \caption{Pressing Test System Setup with Robot Arm and Gripper: The robot arm moves downward slowly, bringing the fingertip of the robotic gripper into contact with the aluminum frame. A six-axis force/torque (FT) sensor, positioned between the robot arm and the flexible wrist, measures the reaction forces at the fingertip and the torque at the universal joint during the interaction.}
    \label{fig:Pressing_Test}
\end{figure}

==> Figure_tex/fig_theoretical_analysis.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
       \includegraphics[width=1.0\textwidth]{Figure/Theoretical_Analysis1.png}
       \caption{}
       \label{fig:Theoretical_Analysis1}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
       \includegraphics[width=1.0\textwidth]{Figure/Theoretical_Analysis2.png}
       \caption{}
       \label{fig:Theoretical_Analysis1}
    \end{subfigure}
    \caption{Free Body Diagram for one module of the flexible wrist}
    \label{fig:Theoretical_Analysis}
\end{figure}

==> Table_tex/table_pickandplace_result.tex <==
\begin{table}[ht]
\centering
\caption{Pick and Place Task Results}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{No.} & \textbf{Object}          & \textbf{Shape} & \textbf{Material} & \textbf{Dims. (mm)}                      & \textbf{Weight(g)} & \textbf{Success Rate \%} \\ \hline
1  & Mustard container      & Irregular  & Plastic   & 80 $\times$ 35 $\times$ 158               & 27.7  & \textbf{100} \\ \hline
2  & Juice container        & Cuboid     & Paper     & 70 $\times$ 70 $\times$ 195               & 40    & \textbf{100} \\ \hline
%3  & Plastic container      & Oval       & Plastic   & 55 $\times$ 31 $\times$ 86                & 46.6  &  \\ \hline
3  & Cup                    & Cylinder   & Plastic   & $\phi$ 75 $\times$ 88                      & 60.7  & \textbf{100} \\ \hline
% 4  & Hot sauce              & Cylinder   & Glass     & 77.5 $\times$ 68.5 $\times$ 170            & 304    &  \\ \hline
4  & Water spray            & Cylinder   & Plastic   & $\phi$ 53 $\times$ 195                      & 90    & \textbf{100} \\ \hline
5  & Shampoo travel kit     & Irregular  & Plastic   & 55 $\times$ 28.5 $\times$ 101              & 113.5 & \textbf{100} \\ \hline
6 & Toothpaste             & Irregular  & Plastic   & 35 $\times$ 160                            & 130   & \textbf{100}  \\ \hline
7 & Tin box                & Cuboid     & Metal     & 71 $\times$ 40 $\times$ 96                 & 140   & \textbf{100} \\  \hline
8 & Sunscreen           & Irregular  & Plastic   & $\phi$ 46 $\times$ 156                      & 154   & \textbf{100} \\  \hline
9 & Red pepper jar         & Cuboid     & Glass     & 43.5 $\times$ 43.5 $\times$ 105             & 155   & \textbf{100} \\  \hline
10 & Pepper container       & Cylinder   & Glass     & $\phi$ 40 $\times$ 157                      & 178   & \textbf{100} \\  \hline
11 & Soap dispenser         & Cylinder   & Plastic   & $\phi$ 44 $\times$ 190                      & 205   & \textbf{100} \\  \hline
12 & Diet coke              & Cylinder   & Metal     & $\phi$ 65 $\times$ 122                      & 250   & \textbf{100} \\  \hline
13 & Tea box                & Cuboid     & Paper     & 77 $\times$ 68 $\times$ 110                            & 371   & \textbf{100} \\  \hline
14 & 500ml Bottle           & Cylinder   & Plastic   & $\phi$ 60 $\times$ 205                      & 508   & \textbf{100} \\  \hline
% 15 & 600ml Bottle           & Cylinder   & Plastic   & $\phi$ 75 $\times$ 295                      & 600   & 0 \\  \hline
15 & 1L Bottle           & Cylinder   & Plastic   & $\phi$ 75 $\times$ 295                      & 1050   &  0 \\ \hline
\multicolumn{6}{|c|}{\textbf{Average}} & \textbf{93.3} \\ \hline
\end{tabular}%
}
\label{tab:pick_and_place_resultse}
\end{table}


==> Table_tex/table_pressing_result.tex <==
\begin{table}[!h]
    \centering
    \renewcommand{\arraystretch}{1.3} % Adjust row height for better readability
    \resizebox{\columnwidth}{!}{ % Adjust the table to fit within one column
    \begin{tabular}{|>{\columncolor[gray]{0.9}\centering\arraybackslash}m{0.2\columnwidth}|
    >{\centering\arraybackslash}m{0.19\columnwidth}|
    >{\centering\arraybackslash}m{0.14\columnwidth}|
    >{\centering\arraybackslash}m{0.14\columnwidth}|
    >{\centering\arraybackslash}m{0.16\columnwidth}|
    >{\centering\arraybackslash}m{0.16\columnwidth}|}
    \hline 
    \rowcolor[gray]{0.9} % Color the first row
    \diagbox[width=8em, height=2.5em]{}{} 
    & \multicolumn{2}{c|}{Buckling Force (N)} 
    & \multicolumn{2}{c|}{Fingertip Deviation (mm)} \\
    \arrayrulecolor{black} % Ensure black line color
    \hline
    \rowcolor[gray]{0.9} % Maintain the grey color for the second row
    & Desired (500g Payload)
    & Measured
    & Max. at Buckling Point
    & Measured \\
    \hline 
    \cellcolor[gray]{0.9}\textbf{Panda} 
    & 8.26 
    & 8.38
    & 10
    & 11.1 \\
    \hline 
    \cellcolor[gray]{0.9}\textbf{BaRiFlex} 
    & 8.2 
    & 7.84
    & 10
    & 14.3 \\
    \hline 
    \cellcolor[gray]{0.9}\textbf{Robotiq} 
    & 12.7 
    & 11.19 $\pm$ 0.46 
    & 10
    & 9.5 $\pm$ 0.3 \\
    \hline
    \end{tabular}
    }
    \caption{Comparison of Force and Fingertip Z-Deviation for different robotic hands during the pressing test. The BaRiFlex fingertip Z-deviation does not include the \SI{3.5}{\milli\meter} compression caused by its material characteristics.}
    \label{tab:pressing_test}
\end{table}

==> Table_tex/table_related_work.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Comparison of Robotic Wrist Designs}
% \label{tab:rw_comparison}
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{l||cccccccc}
% \hline
% \textbf{Wrist} & \textbf{DoF} & \textbf{Actuator Type} & \textbf{Number of Actuator} & \textbf{Stiffness Type} & \textbf{ROM[deg]} & \textbf{Radius and Height[mm]} & \textbf{Weight[g]} \\
% \hline
% Wrist 1  & 3 & Electric & 3 & High        & 40  & 100 / 60    & 70 \\
% Wrist 2  & 3 & Passive & - & Low            & 60      & 70 / 40    & 40 \\
% Wrist 3  & 2 & Pneumatic & 1 & Variable Stiffness   & 120 & 40 / 20 & 20 \\
% Wrist 4 & 2 & Electric  & 3 & Variable Stiffness             & 40      & 30 / 20 & 200 \\
% Ours    & 2 & Passive  & -  & Variable Stiffness  & 50     & 60 / 30  & 80 (Wrist Module: 20g) \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \end{table*}

\begin{table}[ht]
\centering
\caption{Comparison of Robotic Wrist Designs}
\label{tab:rw_comparison}
\begin{tabular}{l|lllllll}
\toprule
\textbf{Author} & \textbf{Year} & \textbf{DoF} & \textbf{Actuators} & \textbf{Stiffness} & \textbf{Radius/Height } & \textbf{Weight} \\
\midrule

Montagnani et al.\cite{montagnani_preliminary_2013}& 2013  & 2 & 1x Servo & Bimodal & 100/60mm & 500g \\

Drigalski et al.~\cite{von_drigalski_0_2020}& 2020 & 6 & 1x Pneumatic & Bimodal & 75/60mm & N/A \\

Zhang et al.~\cite{zhang_stiffness_2020} & 2020 & 2 & 1x Pneumatic & Bimodal & N/A & N/A \\

Milazzo et al.~\cite{milazzo_modeling_2024}& 2024 & 3 & 3x Servo & Contin. & 70/170mm & 1110g \\

Sun et al.~\cite{sun_compact_2025}& 2025 & 2 & 3x Servo & Contin. & 63/55mm & 200g \\

Ours    & 2025 & 2 & - Passive & Bimodal & 60/30mm  & 80g \\
\bottomrule
\end{tabular}
\end{table}

==> table_applied_torque.tex <==
\begin{table}[!h]
    \centering
    \renewcommand{\arraystretch}{1.3} % Adjust row height for better readability
    \resizebox{\columnwidth}{!}{ % Adjust the table to fit within one column
    \begin{tabular}{|>{\columncolor[gray]{0.9}\centering\arraybackslash}m{0.15\columnwidth}|
                        >{\centering\arraybackslash}m{0.18\columnwidth}|
                        >{\centering\arraybackslash}m{0.25\columnwidth}|
                        >{\centering\arraybackslash}m{0.3\columnwidth}|}
    \hline 
    \rowcolor[gray]{0.9} % Maintain the grey color for the second row
    & Length until CoM (mm)
    & Gravitational Force at CoM (N)
    & Estimated Torque for 500g Object (Nm)\\
    \hline 
    \cellcolor[gray]{0.9}\textbf{Panda} 
    & 82.5 
    & 12
    & 0.99 \\
    \hline 
    \cellcolor[gray]{0.9}\textbf{BaRiFlex} 
    & 131 
    & 12.5
    & 1.6\\
    \hline 
    \cellcolor[gray]{0.9}\textbf{Robotiq} 
    & 100 
    & 14.5 
    & 1.45 \\
    \hline
    \end{tabular}
    }
    \caption{The estimated torque when the robotic gripper holds a 500g object at its fingertip.}
    \label{tab:applied_torque}
\end{table}



% \begin{table}[!h]
%     \centering
%     \renewcommand{\arraystretch}{1.3} % Adjust row height for better readability
%     \resizebox{\columnwidth}{!}{ % Adjust the table to fit within one column
%     \begin{tabular}{|>{\columncolor[gray]{0.9}\centering\arraybackslash}m{0.15\columnwidth}|
%                         >{\centering\arraybackslash}m{0.14\columnwidth}|
%                         >{\centering\arraybackslash}m{0.19\columnwidth}|
%                         >{\centering\arraybackslash}m{0.25\columnwidth}|
%                         >{\centering\arraybackslash}m{0.15\columnwidth}|}
%     \hline 
%     \rowcolor[gray]{0.9} % Maintain the grey color for the second row
%     & Length until CoM (mm)
%     & Gravitational Force at CoM (N)
%     & Torque to support 500g Object (Nm)
%     & 10mm Joint angle (degree)\\
%     \hline 
%     \cellcolor[gray]{0.9}\textbf{Panda} 
%     & 82.5 
%     & 12
%     & 0.99
%     & 4.25 \\
%     \hline 
%     \cellcolor[gray]{0.9}\textbf{BaRiFlex} 
%     & 131 
%     & 12.5
%     & 1.6
%     & 2.5\\
%     \hline 
%     \cellcolor[gray]{0.9}\textbf{Robotiq} 
%     & 100 
%     & 14.5 
%     & 1.45 
%     & 3.51\\
%     \hline
%     \end{tabular}
%     }
%     \caption{Comparison of Force and Fingertip Z-Deviation for different robotic hands under with and without screws conditions.}
%     \label{tab:applied_torque}
% \end{table}
